The Procedural Content Generation Benchmark: An Open-source Testbed for Generative Challenges in Games

This paper introduces the Procedural Content Generation Benchmark for evaluating generative algorithms on different game content creation tasks. The benchmark comes with 12 game-related problems with multiple variants on each problem. Problems vary from creating levels of different kinds to creating rule sets for simple arcade games. Each problem has its own content representation, control parameters, and evaluation metrics for quality, diversity, and controllability. This benchmark is intended as a first step towards a standardized way of comparing generative algorithms. We use the benchmark to score three baseline algorithms: a random generator, an evolution strategy, and a genetic algorithm. Results show that some problems are easier to solve than others, as well as the impact the chosen objective has on quality, diversity, and controllability of the generated artifacts.

==> diagrams/benchmark_control.tex <==
\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{%
	\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|}
		\hline
            & \multicolumn{3}{c|}{Random Search} & \multicolumn{3}{c|}{$\mu + \lambda$ Evolution Strategy} & \multicolumn{3}{c|}{Genetic Algorithm} \\\cline{2-10}
		& Q & QC & QCD & Q & QC & QCD & Q & QC & QCD \\
		\hline \hline
           
            Arcade Rules& 9.30$\pm$3.017152& 8.00$\pm$2.431746& 11.90$\pm$1.325503& 2.40$\pm$2.164538& \textbf{100.00}& \textbf{100.00}& 5.00$\pm$3.109038& 81.20$\pm$4.621302& 88.00$\pm$3.439008 \\\hline
            Binary& 8.80$\pm$1.574508& 9.50$\pm$1.400590& 83.70$\pm$6.061099& 18.00$\pm$20.760419& 90.00$\pm$22.621572& \textbf{100.00}& 15.10$\pm$15.381375& 34.00$\pm$16.643902& 50.50$\pm$12.528394 \\\hline
            Building& 3.20$\pm$1.500545& 2.30$\pm$1.014474& \textbf{100.00}& 5.10$\pm$8.937668& 1.50$\pm$2.085606& \textbf{100.00}& 0.70$\pm$1.583510& 22.70$\pm$19.189263& 68.40$\pm$4.438032 \\\hline
            Dangerous Dave& \textbf{0.10}$\mathbf{\pm}$\textbf{0.226216}& 0.00& 0.00& 0.00& 0.00& 0.00& 0.00& 0.00& 0.00 \\\hline
            Elimination& 81.10$\pm$3.880990& 81.30$\pm$2.456174& \textbf{100.00}& 80.00$\pm$30.162096& 90.00$\pm$22.621572& \textbf{100.00}& 81.40$\pm$26.842994& 80.40$\pm$28.840311& 99.20$\pm$1.809726 \\\hline
            The Binding of Isaac& 60.10$\pm$2.063680& 64.10$\pm$1.189875& \textbf{100.00}& 80.00$\pm$30.162096& 70.00$\pm$34.555021& \textbf{100.00}& 30.20$\pm$34.459122& 80.00$\pm$30.162096& \textbf{100.00} \\\hline
            Lode Runner& 3.90$\pm$1.090121& 4.10$\pm$1.141088& 11.00$\pm$1.652046& 8.70$\pm$15.156453& 9.60$\pm$21.716709& 16.50$\pm$21.221585& 12.30$\pm$21.718934& \textbf{16.60}$\mathbf{\pm}$\textbf{25.538230}& 16.20$\pm$24.079669 \\\hline
            Mini Dungeons& 0.00& 0.00& 0.00& 1.30$\pm$2.288397& 21.30$\pm$29.710143& \textbf{50.00}$\mathbf{\pm}$\textbf{37.702619}& 1.60$\pm$1.270752& 8.70$\pm$6.273154& 17.10$\pm$2.533661 \\\hline
            Super Mario Bros& 0.10$\pm$0.226216& 0.10$\pm$0.226216& \textbf{0.70}$\mathbf{\pm}$\textbf{0.482829}& 0.00& 0.00& 0.00& 0.00& 0.00& 0.00 \\\hline
            Sokoban& 23.50$\pm$2.681926& 22.80$\pm$3.068539& \textbf{77.70}$\mathbf{\pm}$\textbf{3.740738}& 25.20$\pm$28.578088& 70.00$\pm$34.555021& 66.80$\pm$30.821839& 5.60$\pm$5.674964& 60.00$\pm$30.084706& 42.40$\pm$30.415897 \\\hline
            Talakat& 0.00& 0.10$\pm$0.226216& 0.30$\pm$0.345550& 0.00& 16.50$\pm$25.573940& \textbf{34.00}$\mathbf{\pm}$\textbf{33.755953}& 0.10$\pm$0.226216& 3.50$\pm$7.669495& 9.20$\pm$9.888154 \\\hline
            Zelda& 0.30$\pm$0.345550& 0.90$\pm$0.626363& 82.00$\pm$6.060630& 5.30$\pm$6.117127& 1.20$\pm$1.422743& \textbf{100.00}& 5.20$\pm$7.324795& 30.30$\pm$12.445520& 49.90$\pm$6.139394 \\\hline

	\end{tabular}%
    }
    \caption{This table shows the number of individuals in the final generation that pass the benchmark criteria for the \textit{controllability} metric for every different problem. The reported value is the mean between 10 runs followed by the 95\% confidence interval.}
    \label{tab:benchmark_control}
\end{table*}


==> diagrams/benchmark_diversity.tex <==
\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{|l||c|c|c|c|c|c|c|c|c|}
            \hline
            & \multicolumn{3}{c|}{Random Search} & \multicolumn{3}{c|}{$\mu + \lambda$ Evolution Strategy} & \multicolumn{3}{c|}{Genetic Algorithm} \\\cline{2-10}
            & Q & QC & QCD & Q & QC & QCD & Q & QC & QCD \\
            \hline \hline
            
            Arcade Rules& 0.70$\pm$0.829458& 1.00$\pm$0.754052& 3.30$\pm$1.817563& 0.90$\pm$0.626363& 0.60$\pm$0.369409& \textbf{99.10}$\mathbf{\pm}$\textbf{2.035941}& 1.00& 1.00& 1.00 \\\hline
            Binary& 98.50$\pm$0.505834& 97.60$\pm$1.477635& 98.50$\pm$0.772674& 19.00$\pm$16.024279& 12.00$\pm$12.440722& \textbf{100.00}& 3.40$\pm$3.906544& 1.10$\pm$0.226216& 33.10$\pm$13.695759 \\\hline
            Building& 91.70$\pm$1.583510& 93.30$\pm$1.471852& \textbf{100.00}& 11.60$\pm$6.310657& 8.00$\pm$6.371631& \textbf{100.00}& 26.20$\pm$9.301474& 21.40$\pm$6.920870& 82.80$\pm$2.282177 \\\hline
            Dangerous Dave& 1.00$\pm$0.584086& 1.70$\pm$0.757813& 0.80$\pm$0.812139& \textbf{80.10}$\mathbf{\pm}$\textbf{29.825513}& 55.70$\pm$34.171222& 77.80$\pm$28.183408& 29.90$\pm$11.383194& 19.50$\pm$14.140242& 34.80$\pm$5.033547 \\\hline
            Elimination& 97.90$\pm$0.856439& 97.80$\pm$1.055673& \textbf{100.00}& 0.10$\pm$0.226216& 0.20$\pm$0.301621& \textbf{100.00}& 1.20$\pm$0.301621& 1.80$\pm$0.564281& 42.00$\pm$12.667182 \\\hline
            The Binding of Isaac& 1.10$\pm$0.626363& 0.70$\pm$0.588934& \textbf{100.00}& 0.00& 0.00& 51.00$\pm$36.696872& 2.60$\pm$0.603242& 3.40$\pm$0.603242& 38.00$\pm$8.928439 \\\hline
            Lode Runner& 0.60$\pm$0.603242& 1.30$\pm$0.956785& 8.30$\pm$1.848582& 1.00$\pm$0.674445& 0.90$\pm$0.920438& \textbf{10.00}$\mathbf{\pm}$\textbf{6.616783}& 1.00& 1.00& 1.00 \\\hline
            Mini Dungeons& 0.60$\pm$0.603242& 0.70$\pm$0.956785& 0.80$\pm$0.657368& \textbf{100.00}& \textbf{100.00}& \textbf{100.00}& 30.20$\pm$2.672368& 29.70$\pm$3.710214& 31.70$\pm$1.753881 \\\hline
            Super Mario Bros& 1.20$\pm$1.000364& 0.70$\pm$0.482829& \textbf{1.80}$\mathbf{\pm}$\textbf{1.000364}& 0.60$\pm$0.691100& 0.90$\pm$0.711372& 0.70$\pm$0.678647& 1.00& 1.00& 1.00 \\\hline
            Sokoban& 1.30$\pm$0.895388& 0.70$\pm$0.678647& 73.00$\pm$5.256778& 80.50$\pm$29.408526& \textbf{89.70}$\mathbf{\pm}$\textbf{22.312944}& 67.20$\pm$30.428233& 31.20$\pm$15.192986& 31.10$\pm$15.097816& 25.70$\pm$15.483066 \\\hline
            Talakat& 0.10$\pm$0.226216& 0.00& 0.20$\pm$0.452431& 9.90$\pm$14.984408& 10.50$\pm$11.382195& \textbf{27.10}$\mathbf{\pm}$\textbf{28.152422}& 2.50$\pm$1.180279& 3.30$\pm$1.583510& 6.90$\pm$4.665994 \\\hline
            Zelda& 68.40$\pm$2.616464& 69.90$\pm$2.007819& 95.30$\pm$1.721157& 62.30$\pm$14.022334& 68.60$\pm$11.985401& \textbf{100.00}& 52.80$\pm$3.827141& 50.10$\pm$10.639623& 80.30$\pm$3.164326 \\\hline

        \end{tabular}%
    }
    \caption{This table shows the number of individuals in the final generation that pass the benchmark criteria for the \textit{diversity} metric for every different problem. The reported value is the mean between 10 runs followed by the 95\% confidence interval.}
    \label{tab:benchmark_diversity}
\end{table*}

==> diagrams/benchmark_quality.tex <==
\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{|l||c|c|c|c|c|c|c|c|c|}
            \hline
            & \multicolumn{3}{c|}{Random Search} & \multicolumn{3}{c|}{$\mu + \lambda$ Evolution Strategy} & \multicolumn{3}{c|}{Genetic Algorithm} \\\cline{2-10}
            & Q & QC & QCD & Q & QC & QCD & Q & QC & QCD \\
            \hline \hline
            
            Arcade Rules& \textbf{100.00$\pm$0.00}& \textbf{100.00$\pm$0.00}& 97.50$\pm$1.59& \textbf{100.00$\pm$0.00}& \textbf{100.00$\pm$0.00}& \textbf{100.00$\pm$0.00}& 52.80$\pm$4.39& 65.60$\pm$6.04& 67.50$\pm$6.99 \\\hline
            Binary& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& \textbf{100.00$\pm$0.00}& \textbf{100.00$\pm$0.00}& \textbf{100.00$\pm$0.00}& 30.60$\pm$5.69& 29.40$\pm$3.02& 26.50$\pm$3.13 \\\hline
            Building& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& \textbf{20.00}$\mathbf{\pm}$\textbf{30.16}& \textbf{20.00}$\mathbf{\pm}$\textbf{29.43}& 0.00$\pm$0.00& 7.30$\pm$5.44& 11.90$\pm$4.73& 0.00$\pm$0.00 \\\hline
            Dangerous Dave& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& 40.70$\pm$36.54& 50.00$\pm$37.70& \textbf{78.20}$\mathbf{\pm}$\textbf{29.76}& 20.40$\pm$13.17& 6.00$\pm$9.07& 28.70$\pm$9.02 \\\hline
            Elimination& 0.00$\pm$0.00& 0.10$\pm$0.23& 0.00$\pm$0.00& 0.00$\pm$0.00& 10.00$\pm$22.621572& \textbf{20.00}$\mathbf{\pm}$\textbf{30.16}& 0.00$\pm$0.00& 8.00$\pm$18.10& 6.80$\pm$15.38 \\\hline
            Isaac& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& 80.00$\pm$30.16& \textbf{90.00}$\mathbf{\pm}$\textbf{22.62}& 27.20$\pm$31.80& 46.40$\pm$2.90& 45.80$\pm$3.28& 0.00$\pm$0.00 \\\hline
            Lode Runner& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00} \\\hline
            Mini Dungeons& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& \textbf{100.00$\pm$0.00}& \textbf{100.00$\pm$0.00}& 78.40$\pm$27.48& 13.40$\pm$1.18& 14.80$\pm$1.96& 13.30$\pm$5.48 \\\hline
            Super Mario Bros& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00}& \textbf{0.00$\pm$0.00} \\\hline
            Sokoban& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& 80.00$\pm$30.16& \textbf{90.00}$\mathbf{\pm}$\textbf{22.62}& 30.00$\pm$34.56& 30.20$\pm$15.193& 30.10$\pm$15.10& 24.70$\pm$15.48 \\\hline
            Talakat& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& 47.60$\pm$36.26& \textbf{60.00}$\mathbf{\pm}$\textbf{36.94}& 40.00$\pm$36.94& 13.00$\pm$10.24& 17.10$\pm$12.28& 14.50$\pm$11.58 \\\hline
            Zelda& 0.00$\pm$0.00& 0.00$\pm$0.00& 0.00$\pm$0.00& 1.10$\pm$0.98& 2.90$\pm$3.15& 0.00$\pm$0.00& \textbf{15.00}$\mathbf{\pm}$\textbf{1.82}& 13.40$\pm$1.36& 0.80$\pm$1.81 \\\hline

        \end{tabular}%
    }
    \caption{This table shows the number of individuals in the final generation that pass the benchmark criteria for the \textit{quality} metric for every different problem. The reported value is the mean between 10 runs followed by the 95\% confidence interval.}
    \label{tab:benchmark_quality}
\end{table*}

==> diagrams/controllability_graphs.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \hspace*{20pt}\includegraphics[width=0.3\linewidth]{images/controllability/legend.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/controllability/quality.pdf}
        \caption{Quality Fitness}
        \label{fig:controllability_q}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/controllability/quality_control.pdf}
        \caption{Quality-Controllability Fitness}
        \label{fig:controllability_qc}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/controllability/quality_control_diversity.pdf}
        \caption{Quality-Controllability-Diversity Fitness}
        \label{fig:controllability_qcd}
    \end{subfigure}
    \caption{Number of runs where the best individual can beat the controllability criteria for each problem across the 10 runs for the 3 baseline algorithms.}
    \label{fig:controllability_graphs}
\end{figure*}

==> diagrams/diversity_graphs.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \hspace*{20pt}\includegraphics[width=0.3\linewidth]{images/diversity/legend.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/diversity/quality.pdf}
        \caption{Quality Fitness}
        \label{fig:diversity_q}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/diversity/quality_control.pdf}
        \caption{Quality-Controllability Fitness}
        \label{fig:diversity_qc}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/diversity/quality_control_diversity.pdf}
        \caption{Quality-Controllability-Diversity Fitness}
        \label{fig:diversity_qcd}
    \end{subfigure}
    \caption{Number of unique individuals according to the problem definition of diversity between the best individual of each one of the 10 separate runs for the 3 baseline algorithms.}
    \label{fig:diversity_graphs}
\end{figure*}

==> diagrams/fitness_graphs.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/arcade.pdf}
        \caption{Arcade Rules}
        \label{fig:fitness_arcade}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/binary.pdf}
        \caption{Binary}
        \label{fig:fitness_binary}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/building.pdf}
        \caption{Building}
        \label{fig:fitness_building}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/ddave.pdf}
        \caption{Dangerous Dave}
        \label{fig:fitness_ddave}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/elimination.pdf}
        \caption{Elimination}
        \label{fig:fitness_elimination}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/isaac.pdf}
        \caption{Isaac}
        \label{fig:fitness_isaac}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/loderunner.pdf}
        \caption{Lode Runner}
        \label{fig:fitness_loderunner}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/mdungeons.pdf}
        \caption{Mini Dungeons}
        \label{fig:fitness_mdungeons}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/smb.pdf}
        \caption{Super Mario Bros}
        \label{fig:fitness_smb}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/sokoban.pdf}
        \caption{Sokoban}
        \label{fig:fitness_sokoban}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/talakat.pdf}
        \caption{Talakat}
        \label{fig:fitness_talakat}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{images/fitness/zelda.pdf}
        \caption{Zelda}
        \label{fig:fitness_zelda}
    \end{subfigure}
    \includegraphics[width=0.3\linewidth]{images/fitness/legend.pdf}
    \caption{Progression of the maximum fitness when optimizing the Quality fitness with the three baseline algorithms. Results are averaged from 10 runs, with 95\% confidence intervals as the shaded area.}
    \label{fig:fitness_graphs}
\end{figure*}

==> diagrams/success_graphs.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \hspace*{20pt}\includegraphics[width=0.3\linewidth]{images/success/legend.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/success/quality.pdf}
        \caption{Quality Fitness}
        \label{fig:success_q}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/success/quality_control.pdf}
        \caption{Quality-Controllability Fitness}
        \label{fig:success_qc}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\linewidth]{images/success/quality_control_diversity.pdf}
        \caption{Quality-Controllability-Diversity Fitness}
        \label{fig:success_qcd}
    \end{subfigure}
    \caption{Number of runs that beat the quality criteria for each problem across the 10 separate runs for the 3 baseline algorithms.}
    \label{fig:success_runs}
\end{figure*}
